Linear Programming Hierarchies in Coding Theory: Dual Solutions

The rate vs. distance problem is a long-standing open problem in coding theory. Recent papers have suggested a new way to tackle this problem by appealing to a new hierarchy of linear programs. If one can find good dual solutions to these LPs, this would result in improved upper bounds for the rate vs. distance problem of linear codes. In this work, we develop the first dual feasible solutions to the LPs in this hierarchy. These match the best-known bound for a wide range of parameters. Our hope is that this is a first step towards better solutions, and improved upper bounds for the rate vs. distance problem of linear codes.

==> archive.tex <==

\begin{proposition}
    Let $f:\cube{rn}\to\R$ be symmetric w.r.t. $\mathfrak{S}_n$,
    i.e. $f(X)=f(Y)$ if $\Gamma_X = \Gamma_Y$. Let $0\neq u\in\cube{r}$, $X\in\cube{r\times n}$
    and $\alpha = \Gamma_X$.
    \[
        (L_{\epsilon_u} * f)(X) = \sum_{v\in\cube{r}} \alpha_v f(\alpha -\epsilon_v +\epsilon_{u+v})
    \]
\end{proposition}
\begin{proof}
    \begin{align*}
        (L_{\epsilon_u} * f)(X)
        &= \sum_{j=1}^{n} f(X+e_j u^\intercal)
    \end{align*}
    Let $v\in\cube{r}$. If the $j$-th column of $X$ is $v$, then
    the matrix $X+e_j u^\intercal$ has one less column of type $v$,
    and one more column of type $u+v$. The number of columns of type
    $v$ in $X$ is $\Gamma_X(v) = \alpha_v$.
\end{proof}

\begin{proposition}
    If $f:\cube{rn}\to\R$ is symmetric under $\mathfrak{G}_r$ then
    \[
        (L_{\epsilon_u} * f)(X) = (L_{\epsilon_{Tu}} * f)(TX)
    \]
    for every $0\neq u\in\cube{r}$ and $T\in\mathfrak{G}_r$.
\end{proposition}
\begin{proof}
    \begin{align*}
        (L_{\epsilon_u} * f)(X)
        &= \sum_{Y} L_{\epsilon_u}(Y) f(X+Y)
        \\
        &= \sum_{j=1}^{n} f(T(X + u e_j^T))
        \\
        &= \sum_{j=1}^{n} f(TX + (Tu) e_j^T))
        \\
        &= (L_{\epsilon_{Tu}} * f)(TX)
    \end{align*}
\end{proof}
\begin{corollary}
    If $f$ is symmetric under $\mathfrak{G}_r$ and $\hat{\phi}_v*f
    \geq \lambda n f$ for some $u$, then 
    $\hat{\phi}_w * f \geq \lambda n f$,
    for every $0\neq w\in\cube{r}$.
\end{corollary}
\begin{proof}
    Let $w = T^\intercal u$.
    \begin{align*}
        (\hat{\phi}_w * f)(X)
        &= \sum_{u: \langle u,w\rangle=1} (A_u+dI)^m f(X) -(n-d)^m f(X)
        \\
        &= \sum_{u: \langle u,T^\intercal v\rangle=1} (A_u+dI)^m f(X) -(n-d)^m f(X)
        \\
        &= \sum_{u: \langle T u, v\rangle=1} (A_u+dI)^m f(X) -(n-d)^m f(X)
        \\
        &= \sum_{u': \langle u', v\rangle=1} (A_{T^{-1}u'}+dI)^m f(X) -(n-d)^m f(X)
        \\
        &= \sum_{u': \langle u', v\rangle=1} (A_{T^{-1}u'}+dI)^m f(X) -(n-d)^m f(X)
        \\
        &= \sum_{u': \langle u', v\rangle=1} (A_{u'}+dI)^m f(TX) -(n-d)^m f(X)
        \\
        &= \sum_{u': \langle u', v\rangle=1} (A_{u'}+dI)^m f(X) -(n-d)^m f(X)
        \\
        &= (\hat{\phi}_v * f)(X)
    \end{align*}
\end{proof}
% \begin{proposition}
%     Let $n,N\in\N$ and let $A_1,\dots,A_n$, $B_1,\dots,B_n$ be 
%     real, symmetric, non-negative, commuting matrices of size $N\times N$.
%     Let $v_1,\dots,v_N$ be mutual the eigenvectors and $Q$ the
%     matrix whose columns are $v_1,\dots,v_N$.
%     Let $f\in\R^N$ such that $f\geq 0$
%     and $Q^\intercal f \geq 0$.
%     Let $p,q$ such that $1/p+1/q = 1$.
%     Then,
%     \begin{equation}
%         \left( \sum_{i=1}^{n} A_i^p \right)^{1/p}
%         \left( \sum_{i=1}^{n} B_i^q \right)^{1/q}
%         f
%         \geq 
%         \left( \sum_{i=1}^{n} A_i B_i \right) f
%         \label{eq:holder_matrices}
%     \end{equation}
%     where the inequalities are component-wise.
% \end{proposition}
% \begin{proof}
%     Denote by $\eig_i(X)$ the $i$-th eigenvector of the matrix $X$,
%     ordered from largest to smallest and counted with multiplicity.
%     Let $\lambda_i = (\eig_i(A_1),\dots,\eig_i(A_n))\in\R^n$
%     and $\gamma_i = (\eig_i(B_1),\dots,\eig_i(B_n))\in\R^n$, for $i=1,\dots,n$.
%     \begin{align*}
%         \left( \sum_{i=1}^{n} A_i^p \right)^{1/p}
%         \left( \sum_{i=1}^{n} B_i^q \right)^{1/q}
%         f
%         = \sum_{i=1}^{N} \lVert \lambda_i \rVert_p
%         \lVert \gamma_i \rVert_q \langle f,v_i\rangle v_i
%     \end{align*}
%     Since $A_i,B_i,f$ are all non-negative, the left-hand side of \eqref{eq:holder_matrices} is non-negative.
%     % The assumption $Q^\intercal f \geq 0$ implies $\langle f,v_i\rangle \geq 0$,
%     So by H\"{o}lder's inequality
%     \[
%         \sum_{i=1}^{N} \lVert \lambda_i \rVert_p
%         \lVert \gamma_i \rVert_q \langle f,v_i\rangle v_i
%         \geq 
%         \sum_{i=1}^{N} \lVert \lambda_i \gamma_i \rVert_1 \langle f,v_i\rangle v_i
%         = \left( \sum_{i=1}^{n} A_i B_i \right) f
%     \]
% \end{proof}
\begin{corollary}
    If $f$ is symmetric under $\mathfrak{G}_r$ and $L_{\epsilon_u}*f
    \geq \lambda n f$ for some $u$, then 
    $L_{\epsilon_{w}} * f \geq \lambda n f$,
    for every $0\neq w\in\cube{r}$.
\end{corollary}

\subsubsection{Christoffel-Darboux for Symmetric Krawtchouks}

We start with standard C-D.
\begin{align*}
    & \binom{n}{\alpha}^{-1}(L_{\epsilon_u}(X) - L_{\epsilon_u}(Y))*
        L_\alpha(X)L_\alpha(Y)
    \\
    &= \binom{n}{\alpha}^{-1}L_\alpha(Y) \sum_{v} (\alpha_{u+v}+1)
        L_{\alpha - \epsilon_v + \epsilon_{u+v}}(X)
    \\
    &- \binom{n}{\alpha}^{-1}L_\alpha(X) \sum_{v} (\alpha_{u+v}+1)
        L_{\alpha - \epsilon_v + \epsilon_{u+v}}(Y)
    \\
    &= \sum_{v}\binom{n}{\alpha}^{-1} (\alpha_{u+v}+1)L_\alpha(Y)
        L_{\alpha - \epsilon_v + \epsilon_{u+v}}(X)
    \\
    &- \sum_{v}\binom{n}{\alpha-\epsilon_v + \epsilon_{u+v}}^{-1}\alpha_{v}
        L_\alpha(X) L_{\alpha - \epsilon_v + \epsilon_{u+v}}(Y)
    \\
    &= \sum_{v}\binom{n}{\alpha}^{-1} (\alpha_{u+v}+1)L_\alpha(Y)
        L_{\alpha - \epsilon_v + \epsilon_{u+v}}(X)
    \\
    &- \sum_{v}\binom{n}{\alpha'}^{-1}(\alpha'+\epsilon_v -\epsilon_{u+v})_{v}
        L_{\alpha'+\epsilon_v -\epsilon_{u+v}}(X) L_{\alpha'}(Y)
    \\
    &= \sum_{v}\binom{n}{\alpha}^{-1} (\alpha_{u+v}+1)L_\alpha(Y)
        L_{\alpha - \epsilon_v + \epsilon_{u+v}}(X)
    \\
    &- \sum_{v}\binom{n}{\alpha'}^{-1}(\alpha'_{u+v}+1)
        L_{\alpha'-\epsilon_v +\epsilon_{u+v}}(X) L_{\alpha'}(Y)
\end{align*}
where $\alpha' = \alpha - \epsilon_v + \epsilon_{u+v}$.
Now consider the sum over $\alpha$ of the same total degree.
\begin{align*}
    &\sum_{|\alpha|=j} \binom{n}{\alpha}^{-1}
        (L_{\epsilon_u}(X) - L_{\epsilon_u}(Y))*
        L_\alpha(X)L_\alpha(Y)
    \\
    &= \sum_{|\alpha|=j}\sum_{v}\binom{n}{\alpha}^{-1}
        (\alpha_{u+v}+1)L_\alpha(Y)
        L_{\alpha - \epsilon_v + \epsilon_{u+v}}(X)
    \\
    &- \sum_{|\alpha|=j}\sum_{v}
        \binom{n}{\alpha'}^{-1}(\alpha'_{u+v}+1)
        L_{\alpha'-\epsilon_v +\epsilon_{u+v}}(X) L_{\alpha'}(Y)
\end{align*}
For every $v\neq 0,u$, $|\alpha'| = |\alpha - \epsilon_v + \epsilon_{u+v}| = |\alpha|$. Thus
\begin{align*}
    &\sum_{|\alpha|=j} \binom{n}{\alpha}^{-1}
        (L_{\epsilon_u}(X) - L_{\epsilon_u}(Y))*
        L_\alpha(X)L_\alpha(Y)
    \\
    &= \sum_{|\alpha|=j}\sum_{v=0,u}\binom{n}{\alpha}^{-1}
        (\alpha_{u+v}+1)L_\alpha(Y)
        L_{\alpha - \epsilon_v + \epsilon_{u+v}}(X)
    \\
    &- \sum_{|\alpha|=j}\sum_{v=0,u}
        \binom{n}{\alpha'}^{-1}(\alpha'_{u+v}+1)
        L_{\alpha'-\epsilon_v +\epsilon_{u+v}}(X) L_{\alpha'}(Y)
    \\
    &= \sum_{|\alpha|=j}\binom{n}{\alpha}^{-1}
        (\alpha_{u}+1)L_\alpha(Y)
        L_{\alpha - \epsilon_0 + \epsilon_{u}}(X)
    \\
    &+ \sum_{|\alpha|=j}\binom{n}{\alpha}^{-1}
        (\alpha_{0}+1)L_\alpha(Y)
        L_{\alpha - \epsilon_u + \epsilon_{0}}(X)
    \\
    &- \sum_{|\alpha|=j}
        \binom{n}{\alpha- \epsilon_0 + \epsilon_{u}}^{-1}(\alpha_{u}+2)
        L_{\alpha-2\epsilon_0 +2\epsilon_{u}}(X) L_{\alpha- \epsilon_0 + \epsilon_{u}}(Y)
    \\
    &- \sum_{|\alpha|=j}
        \binom{n}{\alpha- \epsilon_u + \epsilon_{0}}^{-1}(\alpha_{0}+2)
        L_{\alpha-2\epsilon_u +2\epsilon_{0}}(X) L_{\alpha- \epsilon_u + \epsilon_{0}}(Y)
\end{align*}
\begin{align*}
    &(L_{\epsilon_u}(X) - L_{\epsilon_u}(Y))*\sum_{|\alpha|\leq k} 
    \binom{n}{\alpha}^{-1} L_\alpha(X)L_\alpha(Y)
    \\
    &= \sum_{|\alpha|\leq k} \binom{n}{\alpha}^{-1} 
        L_\alpha(Y) \sum_v (\alpha_{u+v}+1)
            L_{\alpha-\epsilon_v + \epsilon_{u+v}}(X)
    \\
    &- \sum_{|\alpha|\leq k} \binom{n}{\alpha}^{-1} 
        L_\alpha(X) \sum_v (\alpha_{u+v}+1)
            L_{\alpha-\epsilon_v + \epsilon_{u+v}}(Y)
    \\
    &= \sum_{|\alpha|\leq k} \sum_v \binom{n}{\alpha}^{-1} (\alpha_{u+v}+1)
        L_\alpha(Y) 
            L_{\alpha-\epsilon_v + \epsilon_{u+v}}(X)
    \\
    &- \sum_{|\alpha|\leq k} 
        \sum_v \binom{n}{\alpha-\epsilon_v+\epsilon_{u+v}}^{-1}\alpha_{v}
        L_\alpha(X) L_{\alpha-\epsilon_v + \epsilon_{u+v}}(Y)
\end{align*}
In the second sum, replace $\alpha$ with $\alpha -\epsilon_v + \epsilon_{u+v}$,
namely $\alpha' = \alpha -\epsilon_v + \epsilon_{u+v}$.
\begin{align*}
    &= \sum_{|\alpha|\leq k} \sum_v \binom{n}{\alpha}^{-1} (\alpha_{u+v}+1)
        L_\alpha(Y) 
            L_{\alpha-\epsilon_v + \epsilon_{u+v}}(X)
    \\
    &- \sum_{|\alpha'|\leq k} 
        \sum_v \binom{n}{\alpha'}^{-1}(\alpha'+\epsilon_v - \epsilon_{u+v})_{v}
        L_{\alpha+\epsilon_v - \epsilon_{u+v}}(X) L_{\alpha'}(Y)
    \\
    &= \sum_{|\alpha|\leq k} \sum_v \binom{n}{\alpha}^{-1} (\alpha_{u+v}+1)
        L_\alpha(Y) 
            L_{\alpha-\epsilon_v + \epsilon_{u+v}}(X)
    \\
    &- \sum_{|\alpha'|\leq k} 
        \sum_v \binom{n}{\alpha'}^{-1}(\alpha'_v+1)
        L_{\alpha+\epsilon_v - \epsilon_{u+v}}(X) L_{\alpha'}(Y)
\end{align*}
In the second sum, offset $v$ by $u$, i.e. $v'=v+u$.
\begin{align*}
    &= \sum_{|\alpha|\leq k} \sum_v \binom{n}{\alpha}^{-1} (\alpha_{u+v}+1)
        L_\alpha(Y) 
            L_{\alpha-\epsilon_v + \epsilon_{u+v}}(X)
    \\
    &- \sum_{|\alpha'|\leq k} 
        \sum_{v'} \binom{n}{\alpha'}^{-1}(\alpha'_{u+v'}+1)
        L_{\alpha-\epsilon_{v'} + \epsilon_{u+v'}}(X) L_{\alpha'}(Y)
\end{align*}
The sums cancel each other, except for $\alpha,v$ such that
$|\alpha|=k$



Let $U\subset\mathcal{I}_{r,n}$ such that $\alpha \in U \Rightarrow T\alpha \in U$ for every $\alpha\in \mathcal{I}_{r,n}$ and $T\in\Gr{r}$. Define
\[
    f(X,Y) = 
    \sum_{\alpha\in U} \binom{n}{\alpha}^{-1} L_{\alpha}(X)
    \frac{1}{|\Gr{r}|} \sum_{T\in\Gr{r}}  L_{T\alpha}(Y)
\]
Recall that 
\[
    L_{T\alpha}(Y) = \1_{[\Gamma_Y = T\alpha]}
    = \1_{[T^{-1}\Gamma_Y = \alpha]}
    = \1_{[\Gamma_{T^{-1}Y} = \alpha]}
    = L_\alpha(T^{-1}Y)
\]
because
\[
    (T\cdot \Gamma_Y)(u) = \Gamma_Y(T^{-1}u) = \Gamma_{TY}(u)
\]
It is clear that $f(T_1 X,T_2 Y) = f(X,Y)$, because
\begin{align*}
    f(T_1 X,T_2 Y) 
    &= \sum_{\alpha} \binom{n}{\alpha}^{-1} L_{\alpha}(T_1 X)
        \frac{1}{|\Gr{r}|} \sum_{T\in\Gr{r}}  L_{T\alpha}(T_2 Y)
    \\
    &= \sum_{\alpha} \binom{n}{\alpha}^{-1} L_{T_1^{-1}\alpha}(X)
        \frac{1}{|\Gr{r}|} \sum_{T\in\Gr{r}}  L_{T_2^{-1}T\alpha}(Y)
    \\
    &= \sum_{\alpha} \binom{n}{\alpha}^{-1} L_{T_1^{-1}\alpha}(X)
        \frac{1}{|\Gr{r}|} \sum_{T'\in\Gr{r}}  L_{T'\alpha}(Y)
    \\
    &= \sum_{\alpha'} \binom{n}{\alpha'}^{-1} L_{\alpha'}(X)
        \frac{1}{|\Gr{r}|} \sum_{T'\in\Gr{r}}  L_{T'\alpha'}(Y)
\end{align*}
where $T' = T_2^{-1}T$ and $\alpha' = T_1^{-1}\alpha$.

Consider the action of $L_{\epsilon_u}(X) - L_{\epsilon_u}(Y)$ on
$f$. Let $\alpha \in U$ and let $f_{\alpha} = 
\sum_{T_1,T_2\in\Gr{r}} L_{T_1\alpha}(X) L_{T_2\alpha}(Y)$.
\begin{align*}
    (L_{\epsilon_u}(X) - L_{\epsilon_u}(Y))*f_\alpha(X,Y)
    &= \sum_{T_1,T_2\in\Gr{r}} 
    (L_{\epsilon_u}*L_{T_1\alpha})(X) L_{T_2\alpha}(Y)
    \\
    &- \sum_{T_1,T_2\in\Gr{r}} L_{T_1\alpha}(X) 
    (L_{\epsilon_u}*L_{T_2\alpha})(Y)
    \\
    &= \sum_{T_1,T_2\in\Gr{r}} 
    (L_{\epsilon_{T_1u}}*L_{T_1\alpha})(T_1 X) L_{T_2\alpha}(Y)
    \\
    &- \sum_{T_1,T_2\in\Gr{r}} L_{T_1\alpha}(X) 
    (L_{\epsilon_{T_2u}}*L_{T_2\alpha})(T_2Y)
    \\
    &= \sum_{T_1,T_2\in\Gr{r}} L_{T_2\alpha}(Y)
        \sum_{j=1}^{n} L_{T_1\alpha}(T_1 X + T_1 u e_j^\intercal) 
    \\
    &- \sum_{T_1,T_2\in\Gr{r}} L_{T_1\alpha}(X) 
        \sum_{j=1}^{n} L_{T_2\alpha}(T_2 Y + T_2 u e_j^\intercal) 
    \\
    &= \sum_{T_1,T_2\in\Gr{r}} L_{T_2\alpha}(Y)
        \sum_{j=1}^{n} L_{T_1\alpha}(T_1 (X + u e_j^\intercal))
    \\
    &- \sum_{T_1,T_2\in\Gr{r}} L_{T_1\alpha}(X) 
        \sum_{j=1}^{n} L_{T_2\alpha}(T_2 (Y + u e_j^\intercal))
    \\
    &= \sum_{T_1,T_2\in\Gr{r}} L_{T_2\alpha}(Y)
        \sum_{j=1}^{n} L_{\alpha}(X + u e_j^\intercal)
    \\
    &- \sum_{T_1,T_2\in\Gr{r}} L_{T_1\alpha}(X) 
        \sum_{j=1}^{n} L_{\alpha}(Y + u e_j^\intercal)
    \\
    &= |\Gr{r}| \sum_{T\in\Gr{r}} L_{T\alpha}(Y)
        (L_{\epsilon_u}*L_{\alpha})(X)
    \\
    &- |\Gr{r}|\sum_{T \in\Gr{r}} L_{T\alpha}(X) 
        (L_{\epsilon_u}*L_{\alpha})(Y)
    \\
    &= |\Gr{r}| \sum_{T\in\Gr{r}} L_{T\alpha}(Y)
        \sum_{v} (\alpha_v+1)L_{\alpha - \epsilon_v + \epsilon_{u+v}}(X)
    \\
    &- |\Gr{r}|\sum_{T \in\Gr{r}} L_{T\alpha}(X) 
        \sum_{v} (\alpha_v+1)L_{\alpha - \epsilon_v + \epsilon_{u+v}}(Y)
\end{align*}
recall the recurrence relation:
\[
    (L_{\epsilon_u}*L_{\alpha})
    = \sum_{v} (\alpha_v+1)L_{\alpha - \epsilon_v + \epsilon_{u+v}}
\]
and that
\begin{align*}
    \binom{n}{\alpha} \frac{1}{\alpha_u+1}
    &=\frac{1}{\alpha_u+1}
        \binom{n}{\alpha_u}
        \binom{n-\alpha_u}{\alpha_w}
        \binom{n-\alpha_u-\alpha_w}{(\alpha_v)_{v\neq u,w}}
    \\
    &= \frac{1}{n-\alpha_u} \binom{n}{\alpha_u+1} \binom{n-\alpha_u}{\alpha_w}
    \binom{n-\alpha_u-\alpha_w}{(\alpha_v)_{v\neq u,w}}
    \\
    &= \frac{1}{\alpha_w} \binom{n}{\alpha_u+1} \binom{n-(\alpha_u+1)}{\alpha_w-1}
    \binom{n-(\alpha_u+1)-(\alpha_w-1)}{(\alpha_v)_{v\neq u,w}}
    \\
    &= \frac{1}{\alpha_w} \binom{n}{\alpha + \epsilon_u - \epsilon_w}
\end{align*}
so
\begin{align*}
    &\binom{n}{\alpha}^{-1}(L_{\epsilon_u}(X) - L_{\epsilon_u}(Y))*f_\alpha(X,Y)
    \\
    &= \binom{n}{\alpha}^{-1}|\Gr{r}| \sum_{T\in\Gr{r}} L_{T\alpha}(Y)
        \sum_{v} (\alpha_v+1)L_{\alpha - \epsilon_v + \epsilon_{u+v}}(X)
    \\
    &- |\Gr{r}|\sum_{T \in\Gr{r}} L_{T\alpha}(X) 
        \sum_{v} \binom{n}{\alpha+\epsilon_v - \epsilon_{u+v}}^{-1}
            \alpha_{u+v} L_{\alpha - \epsilon_v + \epsilon_{u+v}}(Y)
\end{align*}


\newpage




Define $f$ by the following algorithm.
\begin{enumerate}
    \item f(0) = 1
    \item for $i=1,\dots,n-1$:
    \begin{enumerate}
        \item for $|\alpha| = i$:
        \[
            f(\alpha) = \max\bigg\{0, \max_{0\neq u: \alpha_u \geq 1} \Big\{ 
            (\alpha_0+1)^{-1} \big[
            \lambda n f(\alpha-\epsilon_u)
            - \sum_{v\neq 0}
            (\alpha-\epsilon_u)_v f(\alpha-\epsilon_u - \epsilon_v + \epsilon_{u+v})
            \big]
            \Big\}
            \bigg\}
        \]
    \end{enumerate}
\end{enumerate}
\begin{proposition}
    $f$ is symmetric and well-defined.
\end{proposition}
\begin{proof}
\end{proof}

\begin{proposition}
    There exists a common eigenfunction for $\{K_{\epsilon_u}\}_{0\neq u\in\cube{r}}$.
\end{proposition}
\begin{proof}
    Say $f = \sum_{\alpha} \varphi(\alpha) L_\alpha$.
    Say $\Gamma_X = \alpha$.
    \begin{align*}
        (L_{\epsilon_u} * f)(X)
        &= \sum_{Y} L_{\epsilon_u}(Y) f(X+Y)
        \\
        &= \sum_{j=1}^{n} f(X + u e_j^T)
        \\
        &= \sum_{v\in\cube{r}} \alpha_v \varphi(\alpha - \epsilon_v + \epsilon_{u+v})
    \end{align*}
    We seek $f$ such that 
    \[
        A_u f = L_{\epsilon_u} * f \geq \lambda n f
    \]
    for every $0\neq u\in\cube{r}$.
    Let $f(0) = 1$. 
    
    First note that if $\alpha_j = (n-j)\epsilon_0 + j \epsilon_u$,
    then $(A_u f)(\alpha_j)$ restores the 1-dim. case,
    \[
        (n-j)f((j+1) \epsilon_u)
        + j f((j-1)\epsilon_u) \geq \lambda n f(j \epsilon_u)
    \]
    It is known that by setting 
    \[
        f((j+1) \epsilon_u) = 
        \frac{1}{n-j}(\lambda n f(j \epsilon_u) - j f((j-1)\epsilon_u))
    \]
    for $j=1,\dots,k_0-1$, and $f((j+1) \epsilon_u) = 0$
    for $j \geq k_0$ is a feasible solution.
    
    Now consider $\alpha = j \epsilon_w$.
    \[
        [(A_u - \lambda n I) f ](j\epsilon_w)
        = (n-j) f(j\epsilon_w + \epsilon_u) 
        + j f((j-1)\epsilon_w + \epsilon_{u+w})
        - \lambda n f(j\epsilon_w)
    \]
    Set
    \[
        f(j\epsilon_w + \epsilon_u) 
        = \frac{1}{n-j} \left(
        \lambda n f(j\epsilon_w) - j f((j-1)\epsilon_w + \epsilon_{u+w})
        \right)
    \]
    but if $j = k_0+1$, $f(j\epsilon_w) = 0$ and
    the LHS becomes negative. So set
    
    Order the set $\mathcal{I}_{r,n}$ by decreasing $\alpha_0$,
    i.e. by increasing $|\alpha|$. For $k=1,2,\dots$,
    set $|\alpha|= k$ to
    % For $\alpha\neq 0$,
    % let 
    \[
        \varphi_{\alpha + \epsilon_u}
        = \frac{1}{\alpha_0} \left(\lambda n \varphi_{\alpha}
            - \sum_{0\neq v \in\cube{r}}
                \alpha_v \varphi_{\alpha - \epsilon_v + \epsilon_{u+v}}
        \right)
    \]
    If $\varphi_\alpha <0$ for some $\alpha$, set it to $0$.
\end{proof}
\begin{align*}
    \frac{\varphi_{\alpha + \epsilon_u}}{\varphi_{\alpha}}
    = \frac{1}{\alpha_0} \left(\lambda n 
            - \sum_{0\neq v \in\cube{r}}
                \alpha_v \frac{\varphi_{\alpha - \epsilon_v + \epsilon_{u+v}}}{\varphi_{\alpha}}
        \right)
\end{align*}
\begin{align*}
    \varphi_{\alpha + \epsilon_u}
    - \varphi_{\alpha + \epsilon_{w}}
    &= \frac{1}{\alpha_0} \left(\lambda n \varphi_{\alpha}
            - \sum_{0\neq v \in\cube{r}}
                \alpha_v \varphi_{\alpha - \epsilon_v + \epsilon_{u+v}}
        \right)
    \\
    &- \frac{1}{\alpha_0} \left(\lambda n \varphi_{\alpha}
            - \sum_{0\neq v \in\cube{r}}
                \alpha_v \varphi_{\alpha - \epsilon_v + \epsilon_{w+v}}
        \right)
    \\
    &=  \frac{1}{\alpha_0} \sum_{v\neq 0} \alpha_v 
    \left( \varphi_{\alpha - \epsilon_v + \epsilon_{w+v}}
        - \varphi_{\alpha - \epsilon_v + \epsilon_{u+v}} \right)
\end{align*}
So, as long as $\alpha_0 \geq n/2$,
\begin{align*}
    \Delta_{\alpha,u,w}
    &= \frac{1}{\alpha_0} \left(\lambda n \varphi_{\alpha}
            - \sum_{0,u\neq v \in\cube{r}}
                \alpha_v \varphi_{\alpha - \epsilon_v + \epsilon_{u+v}}
        \right)
    \\
    &- \frac{1}{\alpha_0} \left(\lambda n \varphi_{\alpha}
            - \sum_{0,w\neq v \in\cube{r}}
                \alpha_v \varphi_{\alpha - \epsilon_v + \epsilon_{w+v}}
        \right)
    \\
    &=  \frac{1}{\alpha_0} \sum_{v\neq 0} \alpha_v 
        \Delta_{\alpha-\epsilon_v,u+v,w+v}
    \\
    &\leq \frac{n-\alpha_0}{\alpha_0} \max_{v\neq 0} \Delta_{\alpha-\epsilon_v,u+v,w+v}
\end{align*}
Note that $\varphi_0 = 1$ and $\varphi_{\epsilon_u} = \lambda$
for every $0\neq u\in\cube{r}$.
For $\alpha_0 = n-k$, $k=2,3,\dots,n/2$,
\[
    \Delta_{\alpha,u,w} \leq (1-\lambda)
    \prod_{j=1}^{k} \frac{j}{n-j}
    = (1-\lambda) \frac{k!}{(n-k)!}
\]
Hence
\begin{align*}
    \frac{\varphi_{\alpha + \epsilon_u}}{\varphi_{\alpha}}
    &= \frac{1}{\alpha_0} \left(\lambda n 
        - \sum_{0\neq v \in\cube{r}}
            \alpha_v \frac{\varphi_{\alpha - \epsilon_v + \epsilon_{u+v}}}{\varphi_{\alpha}}
    \right)
    \\
    &= \frac{1}{\alpha_0} \left(\lambda n 
        -\alpha_u \frac{\varphi_{\alpha - \epsilon_u}}{\varphi_\alpha}
        - \sum_{0,u\neq v \in\cube{r}}
            \alpha_v \frac{\varphi_{\alpha} 
            \pm \Delta_{\alpha}
            }{\varphi_{\alpha}}
    \right)
    \\
    &= \frac{1}{\alpha_0} \left(\lambda n 
        -\alpha_u \frac{\varphi_{\alpha - \epsilon_u}}{\varphi_\alpha}
        - (n- \alpha_0 - \alpha_u) \left(1\pm \frac{
            \Delta_{\alpha}
            }{\varphi_{\alpha}}\right)
    \right)
\end{align*}

\newpage
\begin{proof}
    For $\alpha \in \mathcal{I}_{r,n}$, define
    \[
        Q_\alpha = |\mathcal{T}|^{-1} \sum_{T} K_{T\cdot \alpha}
    \]
    the sum is over $T\in\mathcal{T}=GL(r,2)$. Let $u\in\cube{r}$, $T_0\in\mathcal{T}$
    and consider the action of $K_{\epsilon_u}$ and $K_{T_0\cdot (\epsilon_u)} = K_{\epsilon_{T_0^{-1}u}}$ on $Q_\alpha$.
    \begin{align*}
        K_{T_0 \epsilon_{u}} Q_\alpha
        &= |\mathcal{T}|^{-1} \sum_{T} K_{T_0\cdot \epsilon_{u}} K_{T\cdot \alpha}
        \\
        &= |\mathcal{T}|^{-1} \sum_{T} K_{T_0\cdot \epsilon_{u}} K_{T T_0 \alpha}
    \end{align*}
    Recall the recurrence relation:
    \begin{align*}
        K_{\epsilon_u} K_{\alpha}
        &= \sum_{v} (\alpha_v+1) K_{\alpha + \epsilon_v - \epsilon_{v+u}}
    \end{align*}
    \begin{align*}
        K_{T_0 \epsilon_{u}} Q_\alpha
        &= |\mathcal{T}|^{-1} \sum_{T} 
        \sum_{v} (\alpha_v+1) K_{T\alpha + \epsilon_v - \epsilon_{v+T_0^{-1}u}}
        \\
        &= |\mathcal{T}|^{-1} \sum_{T} 
        \sum_{v} (\alpha_v+1) K_{T(\alpha + \epsilon_{Tv} - \epsilon_{Tv+TT_0^{-1}u})}
    \end{align*}
    Let $T' = TT_0^{-1}$, so $T = T'T_0$.
    \begin{align*}
        K_{T_0 \epsilon_{u}} Q_\alpha
        &= |\mathcal{T}|^{-1} \sum_{T'} 
        \sum_{v} (\alpha_v+1) K_{T'T_0(\alpha + \epsilon_{T'T_0v} - \epsilon_{T'T_0v+T'u})}
    \end{align*}
    Let $v' = T_0v$, then $v=T_0^{-1}v'$.
    \begin{align*}
        K_{T_0 \epsilon_{u}} Q_\alpha
        &= |\mathcal{T}|^{-1} \sum_{T'} 
        \sum_{v'} (\alpha_{T_0^{-1}v'}+1) K_{T'T_0(\alpha + \epsilon_{T'v'} - \epsilon_{T'v'+T'u})}
        \\
        &= |\mathcal{T}|^{-1} \sum_{T'} 
        \sum_{v'} (\alpha_{T_0^{-1}v'}+1) K_{T'T_0(\alpha + (T')^{-1}\epsilon_{v'} - (T')^{-1}\epsilon_{v'+u})}
        \\
        &= |\mathcal{T}|^{-1} \sum_{T'} 
        \sum_{v'} (\alpha_{T_0^{-1}v'}+1)
            K_{T'T_0(T')^{-1}(T'\alpha + \epsilon_{v'} - \epsilon_{v'+u})}
        \\
        &= |\mathcal{T}|^{-1} \sum_{T'} 
        \sum_{v'} (\alpha_{T_0^{-1}v'}+1)
            K_{(T'\alpha + \epsilon_{v'} - \epsilon_{v'+u})}\circ(T'T_0(T')^{-1})^T
        \\
        &\vdots
        \\
        &= K_{\epsilon_u} Q_\alpha
    \end{align*}


\end{proof}

Recall Christoffel-Darboux formula:
\begin{align*}
    & (K_{\epsilon_u}(x) - K_{\epsilon_u}(y)) 
        \sum_{\alpha: |\alpha| \leq k}
        \binom{n}{\alpha}^{-1} K_{\alpha}(x) K_{\alpha}(y)
    \\
    &= \sum_{\alpha: |\alpha|=k} \frac{\alpha_u + 1} {\binom{n}{\alpha}}
        \Big[
        K_{\alpha + \epsilon_u}(x) K_{\alpha}(y)
        - K_{\alpha}(x)K_{\alpha + \epsilon_u}(y)
        \Big]
\end{align*}
Assume that $TY = T $ for all $T$.
Apply on the sum over $T$:
\begin{align*}
    & (K_{\epsilon_u}(X) - K_{\epsilon_u}(Y)) |\mathcal{T}|^{-1}\sum_{T}
        \sum_{\alpha: |\alpha| \leq k}
        \binom{n}{T \alpha}^{-1} K_{T \alpha}(X) K_{T \alpha}(Y)
    \\
    &= (K_{\epsilon_u}(X) - K_{\epsilon_u}(Y)) |\mathcal{T}|^{-1}\sum_{T}
        \sum_{\alpha: |\alpha| \leq k}
        \binom{n}{\alpha}^{-1} K_{\alpha}((T^{-1})^T X) K_{\alpha}((T^{-1})^T Y)
    \\
    &= |\mathcal{T}|^{-1}\sum_{T}\sum_{\alpha: |\alpha|=k}
        \frac{\alpha_{u} + 1} {\binom{n}{\alpha}}
        \Big[
        K_{\alpha + \epsilon_u}((T^{-1})^TX) K_{\alpha}((T^{-1})^TY)
        - K_{\alpha}((T^{-1})^T X)K_{\alpha + \epsilon_u}((T^{-1})^TY)
        \Big]
    \\
    &= |\mathcal{T}|^{-1}\sum_{T}\sum_{\alpha: |\alpha|=k}
        \frac{\alpha_{u} + 1} {\binom{n}{\alpha}}
        \Big[
        K_{T(\alpha + \epsilon_u)}(X) K_{T\alpha}(Y)
        - K_{T \alpha}(X)K_{T(\alpha + \epsilon_u)}(Y)
        \Big]
    \\
    &= |\mathcal{T}|^{-1}\sum_{T}\sum_{\alpha: |\alpha|=k}
        \frac{(T^{-1}\alpha)_{u} + 1} {\binom{n}{\alpha}}
        \Big[
        K_{\alpha + T\epsilon_u}(X) K_{\alpha}(Y)
        - K_{\alpha}(X)K_{\alpha + T\epsilon_u}(Y)
        \Big]
    \\
    &= |\mathcal{T}|^{-1}\sum_{T}\sum_{\alpha: |\alpha|=k}
        \frac{\alpha_{Tu} + 1} {\binom{n}{\alpha}}
        \Big[
        K_{\alpha + \epsilon_{T^{-1}u}}(X) K_{\alpha}(Y)
        - K_{\alpha}(X)K_{\alpha + \epsilon_{T^{-1}u}}(Y)
        \Big]
\end{align*}




Apply Fourier transform over $X$:
\begin{align*}
    & (L_{\epsilon_u}(X) - K_{\epsilon_u}(Y)) * |\mathcal{T}|^{-1}\sum_{T}
        \sum_{\alpha: |\alpha| \leq k}
        \binom{n}{T \alpha}^{-1} L_{T \alpha}(X) K_{T \alpha}(Y)
    \\
    &= |\mathcal{T}|^{-1}\sum_{T}\sum_{\alpha: |\alpha|=k}
        \frac{\alpha_{u} + 1} {\binom{n}{\alpha}}
        \Big[
        L_{\alpha + \epsilon_u}((T^{-1})^T X) K_{\alpha}(Y)
        - L_{\alpha}((T^{-1})^T X)K_{\alpha + \epsilon_u}(Y)
        \Big]
\end{align*}



\newpage


\section{Archive}

Let $n\in \N$ and $K_0,K_1,\dots,K_n$ the univariate Krawtchouk polynomials,
orthogonal on the binomial measure $p_j=\binom{n}{j}$, $j=0,\dots,n$.

Let $L_j:\cube{n}\to\{0,1\}$ be the $j$-th level-set indicator, $L_j(x)=\1_{[|x|=j]}$,
for $j=0,\dots,n$ and $x\in\cube{n}$. It is well known that $\hat{L}_j = 2^{-n}K_{j}$.

There exists a function $\Gamma:\cube{n}\to\R$ such that, given $0< \lambda <1$
and $\varepsilon>0$ arbitrarily small,
\begin{enumerate}
    \item $\hat{\Gamma} \geq 0$,
    \item $\hat{\Gamma}(0)>0$
    \item $\hat{L}_1*\hat{\Gamma} \geq \lambda n \hat{\Gamma}$, 
    \item $\hat{\Gamma}$ is supported on $|x|\leq \frac{1}{2}(1-\sqrt{1-\lambda^2})(1+\varepsilon)n$
\end{enumerate}
(see Samorodnitsky - On Delsarte's LP Bounds for Binary Codes)





% Three term relation for Krawtchouk polynomials:
% \[
%     K_1(x)K_{j}(x) = 
%     (j+1)K_{j+1}(x) + (n-j+1)K_{j-1}(x)
% \]
% Christoffel Darboux formula:
% \begin{multline*}
%     (K_1(x)-K_1(y))\sum_{j=0}^{l}\binom{n}{j}^{-1} K_j(x)K_{j}(y)
%     \\
%     = \frac{l+1}{\binom{n}{l}}\left[
%         K_{l+1}(x)K_{l}(y) - K_{l}(x)K_{l+1}(y)
%     \right]
% \end{multline*}
% Second order formula:
% \begin{multline*}
%     (K_1^2(x)-K_1^2(y))\sum_{j=0}^{l}\binom{n}{j}^{-1} K_j(x)K_{j}(y)
%     \\
%     = \frac{(l+1)(l+2)}{\binom{n}{l}}
%     \left[K_{l+2}(x)K_{l}(y) - K_{l}(x)K_{l+2}(y) \right]
%     \\
%     + \frac{(l+1)(n-l+1)}{\binom{n}{l}}
%     \left[K_{l+1}(x)K_{l-1}(y) - K_{l-1}(x)K_{l+1}(y) \right]
% \end{multline*}
% \begin{proof}
%     Multiply C-D by $(K_1(x)+K_1(y))$. The left-hand side
%     is as expeted, while the right-hand side, up
%     to a factor of $\frac{l+1}{\binom{n}{l}}$,
%     \begin{align*}
%         &(K_1(x)+K_1(y))\left[
%         K_{l+1}(x)K_{l}(y) - K_{l}(x)K_{l+1}(y)
%         \right]
%         \\
%         &= K_{l}(y) \left[ (l+2)K_{l+2}(x) + (n-l)K_{l}(x) \right]
%         \\
%         &- K_{l+1}(y) \left[ (l+1)K_{l+1}(x) + (n-l+1)K_{l-1}(x) \right]
%         \\
%         &+ K_{l+1}(x)\left[ (l+1)K_{l+1}(y) + (n-l+1)K_{l-1}(y) \right]
%         \\
%         &- K_{l}(x) \left[ (l+2)K_{l+2}(y) + (n-l)K_{l}(y) \right]
%         \\
%         &= (l+2)\left[K_{l+2}(x)K_{l}(y) - K_{l}(x)K_{l+2}(y) \right]
%         \\
%         &+ (n-l+1)\left[K_{l+1}(x)K_{l-1}(y) - K_{l-1}(x)K_{l+1}(y) \right]
%     \end{align*}
% \end{proof}

% \subsection{Recurrence Relation for Even Krawtchouks}

% \begin{proposition}
%     \[
%         K_2(x) K_{j}(x) = \binom{j+2}{2}K_{j+2} (x)
%         + j(n-j) K_{j}(x)
%         + \binom{n-j+2}{2}K_{j-2}(x)
%     \]
% \end{proposition}
% \begin{proof}
%     For every $x\in\cube{n}$,
%     \begin{align*}
%         (L_2 * L_j)(x)
%         &= \sum_{y}L_2(y)L_j(x+y)
%         \\
%         &= \sum_{1\leq i < j \leq n}L_j(x+e_i +e_j)
%     \end{align*}
%     Assume $L_j(x+e_i +e_j) = 1$. Divide into cases:
%     \begin{itemize}
%         \item If $x_i = x_j = 1$ then $|x+e_i +e_j| = |x|-2$ so $L_{j+2}(x)=1$. There
%         are $\binom{|x|}{2}=\binom{j+2}{2}$ such $i<j$.
%         \item If $x_i=1-x_j$ then $L_j(x) = L_j(x+e_i +e_j) = 1$. The number
%         of such $i<j$ is $|x|(n-|x|) = j(n-j)$.
%         \item If $x_i=x_j=0$ then $|x+e_i+e_j|=|x|+2$ so $L_{j-2}(x)=1$, and there
%         are $\binom{n-|x|}{2}=\binom{n-j+2}{2}$ such $i<j$.
%     \end{itemize}
%     Hence
%     \begin{align*}
%         (L_2 * L_j)(x)
%         &= \binom{j+2}{2} L_{j+2}(x) + j(n-j) L_{j}(x)
%         + \binom{n-j+2}{2} L_{j-2}(x)
%     \end{align*}
%     Apply Fourier transform and use the convolution theorem to complete the proof.
% \end{proof}

% \subsection{Christoffel Darboux Formula for Even Krawtchouks}

% \begin{proposition}
%     \begin{multline*}
%     (K_2(x) - K_2(y)) \sum_{j=0}^{l/2} \binom{n}{2j}^{-1} K_{2j}(x)K_{2j}(y)
%     \\
%     = \frac{\binom{l+2}{2}}{\binom{n}{l}}[ K_{l+2}(x) K_{l}(y) - K_{l}(x) K_{l+2}(y) ]
%     \end{multline*}
% \end{proposition}
% \begin{proof}
%     Let $0\leq j \leq l$ be even and
%     \begin{align*}
%         \binom{n}{j} Q_j(x,y) &= (K_2(x) - K_2(y)) K_{j}(x)K_{j}(y)
%         \\
%         &= K_{j}(y)\left[
%             \binom{j+2}{2}K_{j+2} (x)
%             + j(n-j) K_{j}(x)
%             + \binom{n-j+2}{2}K_{j-2}(x)
%         \right]
%         \\
%         &- K_{j}(x)\left[
%             \binom{j+2}{2}K_{j+2} (y)
%             + j(n-j) K_{j}(y)
%             + \binom{n-j+2}{2}K_{j-2}(y)
%         \right]
%     \end{align*}
%     First, the coefficient of $K_j(x)K_j(y)$ is zero. Second,
%     note that
%     \begin{align*}
%         \binom{n}{j}\frac{1}{(j+1)(j+2)}
%         &= \frac{n!}{(j+2)!(n-j)!}
%         \\
%         &= \frac{n!}{(j+2)!(n-j-2)!}\frac{1}{(n-j-1)(n-j)}
%         \\
%         &= \binom{n}{j+2}\frac{1}{(n-j-1)(n-j)}
%     \end{align*}
%     Let $j' = j+2$.
%     \[
%         \frac{\binom{j+2}{2}}{\binom{n}{j}} K_j(x)K_{j+2}(y)
%         = \frac{\binom{n-j}{2}}{\binom{n}{j+2}} K_j(x)K_{j+2}(y)
%         = \frac{\binom{n-j'+2}{2}}{\binom{n}{j'}} K_{j'-2}(x)K_{j'}(y)
%     \]
%     So
%     \begin{align*}
%         Q_{j}(x,y)
%         &= \frac{\binom{j+2}{2}}{\binom{n}{j}}
%         \left[
%             K_{j+2}(x) K_{j}(y) - K_{j}(x)K_{j+2}(y)
%         \right]
%         \\
%         &- \frac{\binom{j}{2}}{\binom{n}{j-2}}
%         \left[
%             K_{j}(x) K_{j-2}(y) - K_{j-2}(x)K_{j}(y)
%         \right]
%     \end{align*}
%     Summing the $Q_j$ yields the desired result.
% \end{proof}

\section{Analytic Dual Solution}

\subsection{Dual Problem}

Let $\mathcal{D}_0 = \N^{r}\setminus\{\0\}$,
$\mathcal{D}_i = \{(a_1,\dots,a_r)\in\N^r: a_i = 0 \vee d\leq a_i\leq n\}$,
for $i=1,\dots,r$. Let $\mathcal{D} = \bigcap_{i=0}^{r}\mathcal{D}_i$.

\begin{definition}
    The dual of multi-dimensional Delsarte's LP is as follows.
    On the left is the problem on the cube, and on the right its
    symmetric version.
    \begin{align*}
        & \textup{minimize}  && g(0,\dots,0)
            && \bar{g}_{(0,\dots,0)} \\
        & \textup{subject to} && g:\cube{rn}\to\R 
            && \bar{g}: \N^r\to\R \\ 
        &&& g(x_1,\dots,x_r) \leq 0 \quad 
            (|x_1|,\dots,|x_r|) \in \mathcal{D}
            && \bar{g}_\alpha \leq 0 \quad (\alpha_1,\dots,\alpha_r)\in \mathcal{D}
        \\
        &&&\hat{g} \geq 0
            && \sum_{\alpha \in \N^r} \bar{g}_\alpha \prod_{i=1}^{r}K_{\alpha_i} \geq 0
        \\
        &&&\hat{g}(0,\dots,0)=1
            && \sum_{\alpha \in \N^r} \bar{g}_\alpha \prod_{i=1}^{r}K_{\alpha_i}(0) =2^{rn}
    \end{align*}
\end{definition}

\begin{proposition}
    Let $C \subset\cube{n}$ be a code with minimal distance $d$.
    Every feasible solution to the dual problem is
    an upper bound on $|C|^r$.
\end{proposition}
\begin{proof}
    Let $\1_{C}:\cube{n}\to\R$ be the indicator of $C$, let
    $f_C = \frac{2^n}{|C|}\1_C*\1_C$ and
    let $f_{C^r} = f_C \otimes \dots\otimes f_C$ be the tensor
    product of $r$ copies of $f_C$. Then,
    \begin{align*}
        2^{-rn} |C|^r 
        &= \hat{f}_{C^r}(0,\dots,0) \hat{g}(0,\dots,0)
        \\
        &\leq \langle \hat{f}_{C^r}, \hat{g} \rangle_{\mathcal{F}}
        \\
        &= \langle f_{C^r},  g \rangle
        \\
        &\leq 2^{-rn} f_{C^r}(0,\dots,0) g(0,\dots,0)
    \end{align*}
\end{proof}

% \begin{align*}
%     \rho_k^2 = k((n+d)/2-d)^2
%     = k((n-d)/2)^2
%     = k(n-d)^2/4
% \end{align*}

% Let $\theta = (n+d)/2$ and $\rho_k = \sqrt{2k}(\theta - d-1)$, for $k=1,\dots,r$.
% For every $U\subset[r]$, not empty, let
Let $m\in\N$ be even such that $r \leq \left(\frac{1+\delta}{1-\delta}\right)^{m}$.
Define $\phi_U:\cube{rn}\to\R$,
\[
    \phi_U(x_1,\dots,x_r) = 
     -|U|(n-d)^m + \sum_{j\in U}(K_1(x_j) +d)^m
\]
for every $\emptyset \neq U\subset [r]$, and $x_1,\dots,x_r\in\cube{n}$.
\begin{proposition}
    Let $x_1,\dots,x_r \in \cube{n}$ and let $\emptyset\neq U\subset[r]$
    \begin{enumerate}
        \item If $|x_i| \geq d$ for every $i\in U$, then
        $\phi(x_1,\dots,x_r) \leq 0$.
        \item If $x_i = 0$ for some $i\in U$, then 
        $\phi(x_1,\dots,x_r) > 0$.
    \end{enumerate}
\end{proposition}
\begin{proof}
    \hfill
    \begin{enumerate}
        \item If $x\in\cube{n}$ with $|x|\geq d$. Obviously $|x|\leq n$, so
        $(n+d-2x)\in[-n+d,n-d]$, and
        $(K_1(x)+d)^m \leq (n-d)^m$. Hence
        then 
        \[
            \sum_{i\in U} (K_1(x_i)+d)^m  \leq |U| (n-d)^m
        \]
        \item Since $m$ is even,
        \[
            \sum_{i\in U} (K_1(x_i)+d)^m \geq (K_1(0)+d)^m = (n+d)^m \geq r(n-d)^m \geq |U| (n-d)^m
        \]
    \end{enumerate}
\end{proof}

Let $\Phi:\cube{rn}\to\R$,
\[
    \Phi(x_1,\dots,x_r) = \prod_{\emptyset \neq U\subset[r]} \phi_U (x_1,\dots,x_r)
\]
\begin{proposition}
    \hfill
    \begin{enumerate}
        \item $\Phi(0,\dots,0) > 0$.
        \item $\Phi(x_1,\dots,x_r) \leq 0$ for every $(x_1,\dots,x_r) \in \mathcal{D}$.
    \end{enumerate}
\end{proposition}
\begin{proof}
    \hfill
    \begin{enumerate}
        \item Follows directly from the previous proposition.
        \item Let $(x_1,\dots,x_r)\in \mathcal{D}$. For every $i$ such that $x_i=0$,
        every $U\subset[r]$ with $i\in U$, $\phi_U(x_1,\dots,x_r) \geq 0$.
        Let $V = \{1\leq i \leq r: x_i \neq 0\}$. $\Phi(x_1,\dots,x_r) \leq 0$
        if
        \[
            \prod_{\emptyset\neq U \subset V} \phi_U(x_1,\dots,x_r) \leq 0
        \]
        but every factor in the product is non-positive because $|x_i|\geq d$ for every $i\in V$, and there is an odd number of factors, $2^{|V|}-1$.
    \end{enumerate}
\end{proof}

Let $\Gamma_r = \Gamma\otimes \dots \otimes \Gamma$,
the tensor product of $r$ copies of 
$\Gamma$ which was defined
in the preliminaries.

% Define $\Lambda_0:\R\to\R$ by 
% \[
%     \Lambda_0(\xi) = \sum_{j=0}^{l}\binom{n}{j}^{-1}K_{j}(t)K_{j}(\xi)
% \]
% where $l\in\N$ and $0<t\in\R$
% will be determined later. Define $\Lambda:\R^r\to\R$ by
% $\Lambda = \Lambda_0 \otimes \dots \otimes \Lambda_0$.

\begin{thm}
    $g = \Phi\cdot \Lambda^2$ is a feasible solution to the 
    LP. Moreover, it coincides with the MRRW bound.
\end{thm}
\begin{proof}
    First, evidently $g(x_1,\dots,x_r)\leq 0$ if $(|x_1|,\dots,|x_r|)\in\mathcal{D}$.
    
    Let $1\leq j\leq r$ and consider function $\varphi(x) = K_1(x)+d$.
    Choose $\lambda n = (n-2d+\varepsilon)$. Then
    \[
        (\hat{\varphi}+d) * \hat{\Gamma} \geq (n-d+\varepsilon)\hat{\Gamma}
    \]
    which implies
    \[
        (A+d)^m \hat{\Gamma} \geq (n-d+\varepsilon)^m \hat{\Gamma}
    \]
    where $A$ is the adjacency matrix of the $n$-cube.
    And so
    \[
        \hat{\phi}_U*\hat{\Gamma}_r
        \geq (|U|(n-d+\varepsilon)^m -|U|(n-d)^m) \hat{\Gamma}_r
    \]
    choose $\varepsilon$ such that $(n-d+\varepsilon)^m-(n-d)^m)\geq 1$.
    It follows that $\hat{\Phi}*\hat{\Gamma}_r \geq \prod_{j=1}^{r}j^{\binom{r}{j}} \hat{\Gamma}_r$.
    But since $\hat{\Gamma}_r\geq 0$, this implies $\hat{g} \geq 0$.
    
    It remains to evaluate the solution, $g(0)/\hat{g}(0)$.
    \[
        \Phi(0,\dots,0) \leq (rn)^{2^r m}
    \]
    \[
        \hat{g}(0) \geq (r/2)^{2^r} (\hat{\Gamma}_r* \hat{\Gamma}_r)(0,\dots,0)
        = (r/2)^{2^r} \lVert \hat{\Gamma}_r \rVert_2^2
    \]
    \[
        \Gamma_r(0,\dots,0)
        = \langle \1_{supp(\hat{\Gamma}_r)}, \hat{\Gamma}_r \rangle
        \leq \lVert \1_{supp(\hat{\Gamma}_r)}\rVert_2^2  \lVert \hat{\Gamma}_r \rVert_2^2 
    \]
    hence
    \[
        g(0)/\hat{g}(0) \leq (rn)^{2^r m}|supp(\hat{\Gamma}_r)|
        = (rn)^{ \frac{1-\delta}{1+\delta}2^r \log r}|supp(\hat{\Gamma})|^r
    \]
    namely
    \[
        |C| \leq (r/2)^{\frac{1-\delta}{1+\delta}\log r}(2n)^{\frac{1-\delta}{1+\delta}\frac{2^r \log r}{r}}2^{nH(1/2-\sqrt{\delta(1-\delta)})+o(n)}
    \]
    and
    \[
    \mathcal{R}(\delta)
    \leq H\left(1/2-\sqrt{\delta(1-\delta)}\right) + \frac{2^r \log r \log n}{rn}
    \]
    
\end{proof}


